Full-field stress computation from measured deformation fields: a hyperbolic formulation

Recent developments in imaging techniques and correlation algorithms enable measurement of strain fields on a deforming material at high spatial and temporal resolution. In such cases, the computation of the stress field from the known deformation field becomes an interesting possibility. This is known as an inverse problem. Current approaches to this problem, such as the finite element update method, are generally over-determined and must rely on statistical approaches to minimize error. This provides approximate solutions in some cases, however, implementation difficulties, computational requirements, and accuracy are still significant challenges. Here, we show how the inverse problem can be formulated deterministically and solved exactly in two or three dimensions for large classes of materials including isotropic elastic solids, Newtonian fluids, non-Newtonian fluids, granular materials and isotropic plastic solids. This solution is based on a single assumption of the alignment of the principal directions of stress and strain or strain rate. No further assumptions regarding incompressibility, pressure independence, yield surface shape or the hardening law are necessary. This assumption leads to a closed, first order, linear system of hyperbolic partial differential equations with variable coefficients and can be solved to give the solution for any geometry and loading condition. We provide a numerical proof-of-principle study of the plastic deformation of a two-dimensional bar with spatially varying yield stress and strain hardening coefficient. The results are validated indicating the solution is exact up to numerical error. No model calibration or material parameters are required. Interestingly, this solution procedure lends itself to a simple physical interpretation of stress propagation through the material.

==> other_text.tex <==
\section{Assumptions}
\subsection{Plane stress}
\subsection{Plane strain}
\subsection{Neglect elastic strain}
\subsection{Co-directionality hypothesis}
One assumption that may be made to constrain the problem is the co-directionality hypothesis, which is motivated by thermodynamic considerations and supported by experimental data. The assumption is given as follows:



See \cite{Gurtin2010} page 431 for a discussion of thermodynamics, briefly summarized here. The dissipation inequality says that the rate of energy applied to the system must be greater that the energy dissipated and can be summarized by:

\begin{equation}
    \mathbf{T}:\dot{\mathbf{E}} \geq \dot{\psi},
\end{equation}

where $\dot{\psi}$ is the free energy dissipation rate. Then we have

\begin{equation*}
    \dot{\mathbf{E}} = \dot{\mathbf{E^e}} + \dot{\mathbf{E^p}}.
\end{equation*}

We assume that $\mathbf{\dot{E}}$ is deviatoric. Using these assumptions one can deduce that
\begin{equation*}
    \dot{\psi}-\mathbf{T}_0:\dot{\mathbf{E^p}}-\mathbf{T}:\dot{\mathbf{E^e}}\leq 0
\end{equation*}

We assume that the stored energy is elastic:
\begin{equation*}
    \dot{\psi}=\mathbf{T}:\dot{\mathbf{E^e}}
\end{equation*}

This gives rise to the plastic dissipation inequality
\begin{equation}
    D = \mathbf{T}_0:\dot{\mathbf{E^p}}\geq 0.
\end{equation}

We define the norm of a tensor as

\begin{equation}
    |\mathbf{A}| = \sum_i\sum_jA_{ij}^2.
\end{equation}

Note that this will be strictly positive. The dissipation inequality can be expressed as

\begin{equation}
    \frac{\mathbf{T_0}:\dot{\mathbf{E}^p}}{|\mathbf{T_0}||\dot{\mathbf{E}^p|}} = \frac{\mathbf{T_0}:\dot{\mathbf{N}^p}}{|\mathbf{T_0}|} \geq 0,
\end{equation}

where $\mathbf{N^p}=\frac{\mathbf{\dot{E^p}}}{|\mathbf{\dot{E^p}}|}$. The codirectionality hypothesis is as follows:

\begin{equation}
    \frac{\mathbf{T_0}}{|\mathbf{T_0}|} = \frac{\mathbf{\dot{E^p}}}{|\mathbf{\dot{E^p}}|}= \mathbf{N^p}
\end{equation}

This ensures that the dissipation inequality is always satisfied as $\mathbf{N^p}:\mathbf{N^p}\geq0$.

See \cite{Hill1950} figure 8, \cite{Taylor1931}, \cite{Chakrabarty2012} page 84, and references therein for experimental data that supports this. This ensures that (i) the principle directions of the stress and plastic strain tensors are aligned, and (ii) they have have the same sign.

As the elastic strain is neglected, we can directly use the measured strain increment to determine the direction of stress.

The deviatoric stress is given by

\begin{equation}
\mathbf{T_0} = 
\left[
    \begin{matrix}
        \frac{2}{3}T_{11}-\frac{1}{3}T_{22}&T_{12}&0\\
        T_{12}&\frac{2}{3}T_{22}-\frac{1}{3}T_{11}&0\\
        0&0&-\frac{1}{3}(T_{11}+T_{22}\\
    \end{matrix}
    \right]
\end{equation}

\subsection{Governing equations}


\subsection{Discretization}
Consider (\ref{eq:forcex}) for the pixel $i$ steps in the x direction and $j$ steps in the $y$ direction.

\begin{equation}
    T_{xx}^{i+1,j}-T_{xx}^{i-1,j}+T_{xy}^{i,j+1}-T_{xy}^{i,j-1}=0
\end{equation}

